Teacher's pet: understanding and mitigating biases in distillation

Knowledge distillation is widely used as a means of improving the performance of a relatively simple student model using the predictions from a complex teacher model. Several works have shown that distillation significantly boosts the student's overall performance; however, are these gains uniform across all data subgroups? In this paper, we show that distillation can harm performance on certain subgroups, e.g., classes with few associated samples. We trace this behaviour to errors made by the teacher distribution being transferred to and amplified by the student model. To mitigate this problem, we present techniques which soften the teacher influence for subgroups where it is less reliable. Experiments on several image classification benchmarks show that these modifications of distillation maintain boost in overall accuracy, while additionally ensuring improvement in subgroup performance.

==> ensemble.tex <==
Previous work has considered ensembles for improving fairness \cite{EnsembleFairness2019}. 
This motivates a direction for improving fairness of a distilled student by using a teacher which is an ensemble. 

One example of such a direction can be training each model in an ensemble on a subset of labels. The motivation for such way of splitting the data is that it may be challenging to have a single model that works well (and fairly) on all labels.

\subsection{Preliminary experiments}
\label{s:fairness_exp_ensemble}

Training separately on two subsets of classes improves average and worst-class accuracy when evaluated on those subsets. 
Note this is not a fair evaluation, as we assume the knowledge of which subset of classes an example belongs to.

However, when first classifying which subset of classes an example belongs to, and then using the corresponding model trained on a subset of classes, the overall accuracy doesn't improve over a baseline. \href{https://docs.google.com/spreadsheets/d/1J-ws0lqCQ81COtTz1vA5q6srENTnqe6RDlv5Imqt-Gg/edit#gid=0}{spreadsheet}.

\subsection{Next steps}
\begin{itemize}
    \item Is there a way of splitting into subsets of classes that would work better than a random split which we tried? E.g., based on clustering.
    \item We can consider building an ensemble using other criteria than subsets of classes, e.g. by splitting examples in the feature space.
\end{itemize}

\subsection{Related work}

One motivation for using an ensemble is that building one model could potentially lead to using spurious features, whereas when building an ensemble, spurious features from each model could become unimportant upon ensembling. 
\cite{shah2020pitfalls} suggest the individual models trained in an ensemble can still focus on spurious features, which causes ensembles to not be very effective in limiting the focus on spurious features.
It is however not clear if such observation holds in general. Moreover, if it holds, it may be interesting to see whether this issue could be mitigated.

\cite{EnsemblesofLocallyIndependentPredictionModels} trained models for an ensemble by optimizing for diversity on unseen data rather than just on the train data, which improves accuracy and diversity. 
This was accomplished by adding the objective of \emph{orthogonal} classifiers in an ensemble. 


==> header.tex <==
\usepackage{url}

\usepackage{graphicx} %
\usepackage{subfigure} 
\usepackage{multirow}
\usepackage{xcolor}
\usepackage{mathtools}
\usepackage{relsize}
\usepackage{nicefrac}
\usepackage{xspace}
\usepackage{amsmath,amssymb,enumerate}
\usepackage{amsthm,cancel}
\usepackage{natbib}
\usepackage{dsfont}
\usepackage[colorlinks=true,citecolor=blue]{hyperref}
\usepackage[utf8]{inputenc} %
\usepackage[T1]{fontenc}    %
\usepackage[mathscr]{eucal}
\usepackage[inline]{enumitem}

\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{remark}{Remark}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}

\newtheorem*{lemma*}{Lemma}
\newtheorem*{theorem*}{Theorem}
\newtheorem*{assumption*}{Assumption}
\newtheorem*{corollary*}{Corollary}
\newtheorem*{remark*}{Remark}
\newtheorem*{definition*}{Definition}

\newcommand{\resnet}{\textsc{ResNet}}
\newcommand{\bert}{\textsc{Bert}\xspace}


\newcommand{\sag}{\textsc{Sag}}
\newcommand{\sgd}{\textsc{Sgd}\xspace}
\newcommand{\sdca}{\textsc{Sdca}}
\newcommand{\csgd}{\textsc{CSgd}}
\newcommand{\dsgd}{\textsc{DSgd}}
\newcommand{\saga}{\textsc{Saga}}
\newcommand{\stgd}{\textsc{S2gd}}
\newcommand{\svrg}{\textsc{Svrg}\xspace}
\newcommand{\msvrg}{\textsc{Msvrg}}
\newcommand{\gd}{\textsc{GradientDescent}\xspace}
\newcommand{\adagrad}{\textsc{Adagrad}}
\newcommand{\nadam}{\textsc{Nadam}}
\newcommand{\adadelta}{\textsc{Adadelta}}
\newcommand{\adam}{\textsc{Adam}}
\newcommand{\adamnc}{\textsc{AdamNc}}
\newcommand{\adamw}{\textsc{AdamW}}
\newcommand{\rmsprop}{\textsc{RMSprop}}
\newcommand{\amsgrad}{\textsc{AMSGrad}}
\newcommand{\yogi}{\textsc{Yogi}}
\newcommand{\lamb}{\textsc{Lamb}}
\newcommand{\lars}{\textsc{Lars}}
\newcommand{\avsgrad}{\textsc{AVSGrad}}
\newcommand{\cifarnet}{\textsc{Cifarnet}}
\newcommand{\diag}{\text{diag}\xspace}
\newcommand{\sml}[1]{{\small #1}}
\newcommand{\fromto}[3]{\sml{$#1{\;\le\;}#2{\;\le\;}#3$}}

\newcommand{\reals}{\mathbb{R}}
\newcommand{\note}[1]{\textcolor{red}{#1}}
\newcommand{\ip}[2]{\left\langle #1, #2\right\rangle}
\newcommand{\nlsum}{\sum\nolimits}
\newcommand{\Fc}{\mathcal{F}}

\newcommand{\enc}{\textsc{enc}}
\newcommand{\dec}{\textsc{dec}}


\renewcommand{\baselinestretch}{0.97}
\frenchspacing
\sloppy

\usepackage{hyperref}
\usepackage{url}

\usepackage[utf8]{inputenc} %
\usepackage[T1]{fontenc}    %
\usepackage{url}            %
\usepackage{booktabs}       %
\usepackage{amsfonts}       %
\usepackage{nicefrac}       %
\usepackage{microtype}      %
\usepackage{algorithm}
\usepackage{algorithmic}

==> temperature.tex <==
Our first approach to correct distillation is to apply \emph{per-class temperatures}.
To motivate this approach,
recall from Figure~\ref{fig:fair_dist_cifar100_lt_logit_breakdown}
that the teacher logits are highly variable across classes:
{in particular,
the mistakes made by the teacher about ``hard'' classes can be passed to a student and reinforced.}

With this in mind, let us reconsider the common trick of applying temperature scaling to the teacher logits $f^{\mathrm{t}}$,
so that $p^{\mathrm{t}}( y' \mid x ) \propto \exp( T^{-1} \cdot f^{\mathrm{t}}_{y'} ( x ) )$
for some $T > 0$.
The nominal goal of such scaling is to smoothen the teacher predictions,
and prevent them from being overly confident (i.e., close to $0$ or $1$).
Given that the teacher confidences are vastly different across classes, however, applying a uniform scaling is intuitively too coarse-grained.
Ideally, one would like to apply a \emph{class-specific} temperature $p^{\mathrm{t}}( y' \mid x ) \propto \exp( T_y^{-1} \cdot f^{\mathrm{t}}_{y'} ( x ) )$,
for scalars $\{ T_1, \ldots, T_L \}$.

Of course, na\"{i}vely introducing such scalars poses a highly infeasible grid-search for a practitioner.
Intuitively, however,
we would like these temperatures to be larger for classes that are more accurately classified;
we would like to smooth the corresponding predictions more aggressively than classes that are poorly classified,
since we have less confidence in the latter.
To formalise this intuition, we have the following choice of temperatures obtained from a variance-reduction argument.

\begin{theorem}
\label{thm:adaptive-temp}
Consider a binary classification setting, with teacher labels for example $i$ being $y_a^i$ and $y_b^i$. 
Let student temperature per example be $T_i$. 
Let student have marginal preference for the same class ordering as teacher, i.e., if $y^i_a > y^i_b$, then student logits $s^i_a - s^i_b = \delta^i$, for some small positive $\delta^i$. 
Then, as $\delta^i \to 0$, the optimal temperature is $$ T_i^2 \propto y_a -y_b .$$
\end{theorem}

While the above was derived for the binary case,
in multi-class problems,
the natural translation is
$$ T_y^2 \propto \mathbb{E}_{x \mid y}\left[ \left( f_y( x ) \right)^2 - \frac{1}{L - 1} \sum_{y' \neq y} \left( f_{y'}( x ) \right)^2 \right]. $$
As an illustration,
Figure~\ref{fig:fair_dist_cifar100_lt_res56_adaptive_temp}
plots the per-class temperatures versus accuracies for CIFAR-ResNet-56 teacher model on long-tailed version of CIFAR100.
Classes with higher accuracies get higher temperatures,
so that they are smoothed more when employed by the student.

\begin{figure}
    \centering
    \resizebox{0.7\linewidth}{!}{\includegraphics[scale=0.5]{figs/fair_dist_cifar100_lt_res56_adaptive_temp.pdf}}
    \caption{Plot of per-class temperatures versus accuracies for CIFAR-ResNet-56 teacher model on CIFAR-100-LT.
    Classes with higher accuracies get higher temperatures,
    so that they are smoothed more when employed by the student.
    }
    \label{fig:fair_dist_cifar100_lt_res56_adaptive_temp}
\end{figure}

